Cross-Lingual Document Retrieval with Smooth Learning

Cross-lingual document search is an information retrieval task in which the queries' language differs from the documents' language. In this paper, we study the instability of neural document search models and propose a novel end-to-end robust framework that achieves improved performance in cross-lingual search with different documents' languages. This framework includes a novel measure of the relevance, smooth cosine similarity, between queries and documents, and a novel loss function, Smooth Ordinal Search Loss, as the objective. We further provide theoretical guarantee on the generalization error bound for the proposed framework. We conduct experiments to compare our approach with other document search models, and observe significant gains under commonly used ranking metrics on the cross-lingual document retrieval task in a variety of languages.

==> preliminary.tex <==
% In this section, we formulate the problem of Smooth Neural Ordinal Regression for Search. 
For each query $\bm{q}$ from language $A$, we are given a set of documents $\bm{D} = (D_1, D_2, ..., D_m)$ from a different language $B$ and the degrees of \textit{relevance} $\bm{y} \in \mathbbm{R}^m$, where the entries in $\bm{y}$ typically belongs to ordered class $\{1, ..., K\}$. The goal of Learning-to-rank is to return an ordered or unordered subset of documents $\bm{D}$, depending on the evaluation metrics, which are more relevant to the query. Most common evaluation metrics, such as NDCG and Precision, however, are discontinuous and thus cannot be directly optimized. As a result, researchers usually assume an unknown continuous relevance score $r$, where a higher value $r$ means a larger $y$ and higher relevance between the query and the document. To optimize the model, one typically minimizes the \textit{surrogate} loss function that is easier to optimize using the relevance score $r$, after which a subset of the documents are being chosen by ordering their relevance score from high to low. 
% In the next section, we will discuss the model to estimate $r$ and the loss functions to optimize the model.  

